Swept-Angle Synthetic Wavelength Interferometry

We present a new imaging technique, swept-angle synthetic wavelength interferometry, for full-field micron-scale 3D sensing. As in conventional synthetic wavelength interferometry, our technique uses light consisting of two narrowly-separated optical wavelengths, resulting in per-pixel interferometric measurements whose phase encodes scene depth. Our technique additionally uses a new type of light source that, by emulating spatially-incoherent illumination, makes interferometric measurements insensitive to aberrations and (sub)surface scattering, effects that corrupt phase measurements. The resulting technique combines the robustness to such corruptions of scanning interferometric setups, with the speed of full-field interferometric setups. Overall, our technique can recover full-frame depth at a lateral and axial resolution of 5 microns, at frame rates of 5 Hz, even under strong ambient light. We build an experimental prototype, and use it to demonstrate these capabilities by scanning a variety of objects, including objects representative of applications in inspection and fabrication, and objects that contain challenging light scattering effects.

==> conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

We presented a technique for depth sensing at micron-scale spatial and axial resolutions. Our technique, \name synthetic wavelength interferometry, combines the complementary advantages of full-field interferometry (high speed, pixel-level spatial resolution) and scanning interferometry (robustness to global illumination). 
%uses light comprising two narrowly-separated optical wavelengths. We showed that the envelope of per-pixel interferometric measurements in such a setup is a sinusoid that depends inversely upon the separation between the wavelengths, and whose phase encodes the depth of the pixel. We added a \name scanning mechanism that provides pixel-level robustness to global illumination. Finally, we proposed filtering interferometric measurements with an ambient light image of the scene to preserve high-resolution features in the estimated depth.
We demonstrated the advantages of our technique by capturing high-quality depth measurements for a variety of scenes with fine spatial features, facing challenges from complicated light transport effects such as interreflections, subsurface scattering, specularities. We validated the micrometer axial resolution of our technique by estimating the numerical accuracy of estimated depth, and showed the robustness of our technique to ambient illumination. We expect that these results will facilitate applications of \name synthetic wavelength interferometry in areas such as computer vision, biomedical imaging, and industrial fabrication. In addition, we hope that our work will motivate future research on improved techniques for phase unwrapping and robust depth reconstruction from interferometry data.

==> renderings.tex <==
\section{3D renderings of measured depths}
In Figure~\ref{fig:microscopic_renderings} and Figure~\ref{fig:macroscopic_renderings}, we render the depths recovered with our
technique in Figures~6 and 7 of the main paper respectively.
\begin{figure*}
\centering
\includegraphics[scale=0.9]{figures/microscopic-renderings.pdf}
\caption{Recovered depths for scenes with microscopic depth ranges rendered as surfaces. From left to right:
ambient light image,
one of our raw images,
depth measured using OCT,
our depth with bilateral filtering and direct-only probing,
our depth with Gaussian filtering and direct-only probing,
our depth with Gaussian filtering and no probing.
}
\label{fig:microscopic_renderings}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[scale=0.96]{figures/macroscopic-renderings.pdf}
\caption{Depth reconstruction results for scenes with macroscopic depth ranges rendered as
surfaces. From left to right:
ambient light image,
one of our raw images,
depth measured using OCT,
our depth with bilateral filtering and direct-only probing,
our depth with Gaussian filtering and direct-only probing,
our depth with Gaussian filtering and no probing.
}
\label{fig:macroscopic_renderings}
\end{figure*}


==> teaser.tex <==
\begin{figure*}[!ht]
\centering
\includegraphics{figures/teaser.pdf}
\vspace*{-20pt}
\caption{\textbf{Reconstructing the eagle embossed on a United States twenty-dollar bill}. The features on the eagle are raised \unit[20]{\textmu m} off the surface of the bill. From left to right: location of the eagle on the bill, an ambient light image of the eagle, a raw frame captured by our method,  the depth recovered by our method rendered as a surface, and  plotted as a depth map. The state-of-the-art technique, optical coherence tomography, requires twenty times as many measurements as our method does to capture a depth map of comparable quality.}
\label{fig:teaser}
\end{figure*}

